Regrading Policies for Flexible Information Flow Control in Session-Typed Concurrency

Noninterference guarantees that an attacker cannot infer secrets by interacting with a program. Information flow control (IFC) type systems assert noninterference by tracking the level of information learned (pc) and disallowing communication to entities of lesser or unrelated level than the pc. Control flow constructs such as loops are at odds with this pattern because they necessitate downgrading the pc upon recursion to be practical. In a concurrent setting, however, downgrading is not generally safe. This paper utilizes session types to track the flow of information and contributes an IFC type system for message-passing concurrent processes that allows downgrading the pc upon recursion. To make downgrading safe, the paper introduces regrading policies. Regrading policies are expressed in terms of integrity labels, which are also key to safe composition of entities with different regrading policies. The paper develops the type system and proves progress-sensitive noninterference for well-typed processes, ruling out timing attacks that exploit the relative order of messages. The type system has been implemented in a type checker, which supports security-polymorphic processes using local security theories.

==> figs/LR-ext.tex <==
\begin{figure*}
    % \begin{small}
     %
     \small
     \begin{mathpar}
     \begin{array}{lll}
    (l_{\&}) &  (\mc{D}_1;\mc{D}_2) \in \mathcal{V}^\xi_{ \Psi_0}\llbracket \Delta, y_\alpha{:}\&\{\ell{:}A_\ell\}_{\ell \in I}\langle c, e \rangle \Vdash K \rrbracket_{\cdot; y^\alpha}^{m+1}\\
    & \m{iff} \quad 
    \quad
     (\mc{D}_1;\mc{D}_2) \in \m{Tree}_{\Psi_0}(\Delta, y_\alpha{:}\&\{\ell{:}A_\ell\}_{\ell \in I}\langle c, e \rangle \Vdash K)\, \m{and}\, \exists k_1,k_2 \in I.  (c \sqsubseteq \xi \rightarrow k_1=k_2)\, \m{and}\,\\
    &\;\quad \qquad \mathcal{D}_1=\mathbf{msg}( y_\alpha^{\langle c, e \rangle}.k_1) \mathcal{D}'_1 \, \m{and}\ \mathcal{D}_2=\mathbf{msg}( y_\alpha^{\langle c, e \rangle}.k_2)\mathcal{D}'_2\,  \,\m{and} \\
   &\;\quad \qquad ( \mc{D}'_1; \mc{D}'_2)
    \in  \mathcal{E}^\xi_{ \Psi_0}\llbracket \Delta, y_{\alpha+1}{:}A_{k_1}{\langle c, e \rangle} \Vdash K \rrbracket^{m}   \\

    (r_{\&}) &(\mc{D}_1;\mc{D}_2) \in \mathcal{V}^\xi_{ \Psi_0}\llbracket \Delta \Vdash y_\alpha{:}\&\{\ell{:}A_\ell\}_{\ell \in I}\langle c,e \rangle\rrbracket_{y^\alpha; \cdot}^{m+1} \\
    &\;\m{iff} \quad \quad
    %c \sqsubseteq e \,\m{and}\,
    (\mc{D}_1;\mc{D}_2) \in \m{Tree}_{\Psi_0}(\Delta \Vdash y_\alpha{:}\&\{\ell{:}A_\ell\}_{\ell \in I}\langle c,e \rangle)\,\m{then}\forall k_1, k_2 \in I. \m{if}\, (c \sqsubseteq \xi \rightarrow k_1=k_2)\,  \m{then}\,\\
    &\; \quad \qquad  (\mc{D}_1 \mathbf{msg}( y_\alpha^{\langle c,e \rangle}.k_1) , \mc{D}_2\mathbf{msg}( y_\alpha^{\langle c,e \rangle}.k_2))\in  \mathcal{E}^\xi_{\Psi_0}\llbracket \Delta \Vdash y_{\alpha+1}{:}A_{k_1}\langle c,e \rangle\rrbracket^{m}\\[2pt]
   \end{array}
     \end{mathpar}
     %
    % \end{small}
    \vspace{-5pt}
     \caption{Value interpretation of logical relation for \emph{left} and \emph{right} communications of external choice ($\&$).}
     \vspace{-5pt}
     \label{fig:rel_value_ext}
     \end{figure*}
 
 
    
         

==> figs/LR-term.tex <==
\begin{figure*}
    {\small
    \[\begin{array}{lcl}
        ({\mc{B}_1}, {\mc{B}_2}) \in \mc{E}^\xi_{ \Psi_0}\llbracket \Delta \Vdash K \rrbracket^{m+1} \qquad
        \m{iff} \\[2pt]
       \quad  (\mc{D}_1;\mc{D}_2)\in \m{Tree}_{\Psi_0}(\Delta \Vdash K)\,\m{and} \forall \,\Upsilon_1,\, \Theta_1, \, \mc{D}'_1.\,\m{if}\; \mc{D}_1\mapsto^{{*}_{\Upsilon_1; \Theta_1}} \; \mc{D}'_1\,  \m{then}\\
        \quad \exists\, \Upsilon_2\,\mc{D}'_2.\, \m{\,such \, that\,}\,\mc{D}_2\mapsto^{{*}_{ \Upsilon_2}}\mc{D}'_2 \; \m{and}\; \Upsilon_1 \subseteq \Upsilon_2\, \m{and}\\
        \quad \forall\, y_\alpha \in \mb{Out}(\Delta \Vdash K).\, \mb{if}\, y_\alpha \in \Upsilon_1.\, \mb{then}\, ({\mc{D}'_1}; {\mc{D}'_2})\in \mc{V}^\xi_{\Psi_0}\llbracket  \Delta \Vdash K \rrbracket_{\cdot;y_\alpha}^{m+1}\,\m{and}\,\\[2pt]
        \quad \forall\, y_\alpha \in \mb{In}(\Delta \Vdash K). \mb{if}\, y_\alpha \in \Theta_1.\, \mb{then}\, ({\mc{D}'_1}; {\mc{D}'_2})\in \mc{V}^\xi_{\Psi_0}\llbracket  \Delta \Vdash K \rrbracket_{y_\alpha;\cdot}^{m+1}    %\\[4pt]
   
    % ({\mc{B}_1}, {\mc{B}_2}) \in \mc{E}^\xi_{ \Psi_0}\llbracket \Delta \Vdash K \rrbracket^{0} &
    % \m{iff}&
    % \mc{B}_1=\mc{C}_1\mc{D}_1\mc{F}_1 \,\m{and}\,\mc{B}_2=\mc{C}_2\mc{D}_2\mc{F}_2\,\m{and}\,(\lr{\mc{C}_1}{\mc{D}_1}{\mc{F}_1}; \lr{\mc{C}_2}{\mc{D}_2}{\mc{F}_2})\in \m{Tree}_{\Psi_0}(\Delta \Vdash K)
        \end{array}\]
    }
    \vspace{-5pt}
    \caption{Term interpretation of logical relation (the inductive case).}
    \vspace{-5pt}
    \label{fig:rel_term_1}
    \end{figure*}
    

==> sections-arxiv/implementation.tex <==
We implemented a \emph{type checker} for $\lang$ in OCaml.
The type checker uses a different syntax from the more formal one used in this paper;
deviations are explained in TR-\secref{apx:implementation}.
% The implementation uses a standard \emph{forward} process.

{\bf User-specified security semilattice.} Our type checker allows the user to specify a 
concrete security join-semilattice $\Psi_0$, such as our banking example lattice, (see \defref{apx:def:lattice} on \pagref{apx:def:lattice} in the TR) and verify its validity.
It will reject security levels that fail the semilattice axioms.
To specify $\Psi_0$, the user includes a
\texttt{secrecy} section, listing the elements of the lattice in decreasing order of secrecy.

{\bf Lattice theories for polymorphic process definitions.} Our type checker allows the programmer 
to specify any number of \emph{lattice theories}, as defined in \defref{apx:def:lattice} on \pagref{apx:def:lattice} in the TR.
A lattice theory postulates a series of security terms $c, d \in \mc{S}$,
ranging over the elements of the concrete security lattice as well as a set of security variables $\psi \in \mathcal{V}$,
along with a list of relations $E \in \mathcal{E}$ that the variables must satisfy.
According to \defref{apx:def:lattice}, $E$ may only be of the form $c \sqsubseteq d$,
but the implementation also allows programmers to specify 
equality between formulas (\eg $c \sqcup d = e \sqcup \texttt{Alice}$), 
which is desugared into two $\sqsubseteq$ relations 
($c \sqcup d \sqsubseteq e \sqcup \texttt{Alice}$, and vice versa). Lattice theories are named.
%
A process is then parametrized over a lattice theory of the programmer's choice.

{\bf Mutual recursive definition.} The type checker also implements limited support for 
equi-recursive definitions, in line with the rules in \Cref{fig:config-typing}.

{\bf Synchronization pattern check.} The type checker implements the pattern checks described 
in \Cref{sec:sync-patterns}. It will first attempt to apply the unsynchronized rules.
% If any of the rules apply, the type checker commits to that choice.
If none of the rules apply, the type checker attempts to apply the synchronized rules,
rejecting the program when this fails.
This algorithm is fine because the unsynchronized rules are \emph{invertible}.

